Statistical Estimation of Confounded Linear MDPs: An Instrumental Variable Approach

In an Markov decision process (MDP), unobservable confounders may exist and have impacts on the data generating process, so that the classic off-policy evaluation (OPE) estimators may fail to identify the true value function of the target policy. In this paper, we study the statistical properties of OPE in confounded MDPs with observable instrumental variables. Specifically, we propose a two-stage estimator based on the instrumental variables and establish its statistical properties in the confounded MDPs with a linear structure. For non-asymptotic analysis, we prove a $\mathcal{O}(n^{-1/2})$-error bound where $n$ is the number of samples. For asymptotic analysis, we prove that the two-stage estimator is asymptotically normal with a typical rate of $n^{1/2}$. To the best of our knowledge, we are the first to show such statistical results of the two-stage estimator for confounded linear MDPs via instrumental variables.

==> tex/semieffi.tex <==
In this section, we study the semiparametric efficiency bound of confounded MDPs with instrumental variables. Firstly, we define the semiparametric model as:
\begin{defn}
Under assumption $z\indep\varepsilon|(s,a)$, the semiparametric model lies in:
\begin{align*}
    \FM=\big{\{}&p(s,a,s',z,\varepsilon)=p_{z}(z)p_{s,a|z}(s,a|z)p_{\varepsilon|s,a}(\varepsilon|s,a)p_{s'|s,a}(s'|s,a):\\
    &\varepsilon=r-\bm{\phi}(s,a)^\top\bm{\omega},\hspace{2pt} p_{s'|s,a}(s'|s,a)=\bm{\phi}(s,a)^\top\bm{\nu}(s'), \hspace{2pt}\EB[\varepsilon|z]=0\big{\}},
\end{align*}
where $\EB[\varepsilon|z]=\sum_{s\in\SM,a\in\AM}\int\varepsilon p_{\varepsilon|s,a}(\varepsilon|s,a)p_{s,a|z}(s,a|z)d\varepsilon$.
\end{defn}
In the following, we drop the subscript to ease the symbols and denote the true model as $\bm{\omega}_0$ and $\bm{\nu}_0(s')$. We can show the tangent space of $\FM$ is:
\begin{thm}
    \label{thm: tangent}
    The tangent space of $\FM$ is given by:
    \begin{align*}
        \Lambda_{\FM}=\Big{\{} &g(s,a,z,\varepsilon)+\frac{\bm{\phi}(s,a)^\top\bm{\dot\nu}(s')}{\bm{\phi}(s,a)^\top\bm{\nu}_0(s')}:\sum_{s'} \bm{\dot\nu}(s')=\bm{0}_d, \EB g(s,a,z,\varepsilon)=0,\\
        &\EB[\varepsilon g(s,a,z,\varepsilon)|z]=\bm{c}^\top\EB[\bm{\phi}(s,a)|z]\text{ for some $\bm{c}\in\RB^d$}\Big{\}}\cap \LM_2^0.
    \end{align*}
\end{thm}
And we also can find an influence function $\psi$:
\begin{align*}
    \psi(s,a,s',z,\varepsilon)=\frac{1}{1-\gamma}\frac{d_{\pi^e}(s,a)}{p(s,a,z)}\left(r+\gamma V_{\pi^e}(s')-Q_{\pi^e}(s,a)\right),
\end{align*}
where we can prove $\psi$ is mean zero. Thus we can project $\psi$ onto $\FM$ to obtain the efficient influence function $\psi_{\text{eff}}$:
\begin{thm}
    \label{thm: efi}
    The efficient influence function     for estimating $V_{\pi^e}(\mu)$ is:
    \begin{align*}
        \psi_{\text{eff}}(s,a,s',z,\varepsilon)=&\psi_{\text{eff},1}(s,a,z,\varepsilon)+\psi_{\text{eff},2}(s,a,z,s'),\\
        \psi_{\text{eff},1}(s,a,z,\varepsilon):=&\frac{1}{1-\gamma}\frac{d_{\pi^e}(s,a)}{p(s,a,z)}(\varepsilon-\EB[\varepsilon|s,a])-\frac{\EB_{d_{\pi^e}}\var(\varepsilon|s,a)}{(1-\gamma)p(z)}\Omega(z)^{-1}\varepsilon\\
        &+\frac{\EB_{d_{\pi^e}}\var(\varepsilon|s,a)}{1-\gamma}\EB_{\Omega^{-1}}[\bm{\phi}_{\rho}(z)^\top]\bm{V}^{-1}\bm{\phi}_{\rho}(z)\Omega(z)^{-1}\varepsilon,\\
        \psi_{\text{eff},2}(s,a,z,s'):=&\frac{\gamma}{1-\gamma}\EB_{d_{\pi^e}}[\bm{\phi}(s,a)^\top]\left[V_{\pi^e}(s')-\left(\EB_{\bm{\Delta}^{-1}}V_{\pi^e}(s')\right)\left(\EB_{\bm{\Delta}^{-1}}\mathbbm{1}\right)^{-1}\right]\frac{\bm{\Delta}(s')^{-1}\bm{\phi}(s,a)}{\bm{\phi}(s,a)^\top\bm{\nu}_0(s')},
    \end{align*}
    where $\Omega(z)=\var(\varepsilon|z),\bm{V}=\EB[\bm{\phi}_{\rho}(z)\Omega(z)^{-1}\bm{\phi}_{\rho}(z)^\top], \bm{\Delta}(s')=\sum_{s\in\SM,a\in\AM}p(s,a)\frac{\bm{\phi}(s,a)\bm{\phi}(s,a)^\top}{\bm{\phi}(s,a)^\top\bm{\nu}_0(s')}$. The variance of $\psi_{\text{eff}}$ is:
    \begin{align*}
        \var(\psi_{\text{eff}})=&\var(\psi_{\text{eff},1})+\var(\psi_{\text{eff},2}),\\
        \var(\psi_{\text{eff},1}):=&\frac{1}{(1-\gamma)^2}\sum_{s,a,z}\frac{d_{\pi^e}(s,a)^2}{p(s,a,z)}\var(\varepsilon|s,a)\\
        &+\frac{(\EB_{d_{\pi^e}}\var(\varepsilon|s,a))^2}{(1-\gamma)^2}\left(\EB_{\Omega^{-1}}[\bm{\phi}_{\rho}(z)^\top]\bm{V}^{-1}\EB_{\Omega^{-1}}[\bm{\phi}_{\rho}(z)]-\EB_{\Omega^{-1}}p(z)^{-1}\right),\\
        \var(\psi_{\text{eff},2}):=&\frac{\gamma^2}{(1-\gamma)^2}\EB_{d_{\pi^e}}[\bm{\phi}(s,a)^\top]\left[\EB_{\bm{\Delta}^{-1}}V_{\pi^e}(s')^2-\EB_{\bm{\Delta}^{-1}}V_{\pi^e}(s')\left(\EB_{\bm{\Delta}^{-1}}\mathbbm{1}\right)^{-1}\EB_{\bm{\Delta}^{-1}}V_{\pi^e}(s')\right]\EB_{d_{\pi^e}}[\bm{\phi}(s,a)].
    \end{align*}
\end{thm}

\begin{rem}
    Here we give an explicitly rough bound on $\var(\psi_{\text{eff},2})$. For any vector $\bm{\alpha}\in\RB^d$ and $\|\bm{\alpha}\|_2=1$, we have
    \begin{align*}
        \bm{\alpha}^\top\bm{\Delta}(s')\bm{\alpha}&=\sum_{s\in\SM,a\in\AM}\frac{p(s,a)}{p(s'|s,a)}[\bm{\phi}(s,a)^\top\bm{\alpha}]^2\\
        &\overset{(a)}{\ge}\frac{(\sum_{s\in\SM,a\in\AM}p(s,a)[\bm{\phi}(s,a)^\top\bm{\alpha}]^2)^2}{\sum_{s\in\SM,a\in\AM}p(s'|s,a)p(s,a)[\bm{\phi}(s,a)^\top\bm{\alpha}]^2}\\
        &\overset{(b)}{\ge}\frac{\underline{\sigma}^2}{\sum_{s\in\SM,a\in\AM}p(s'|s,a)p(s,a)[\bm{\phi}(s,a)^\top\bm{\alpha}]^2}\\
        &\ge\frac{\underline{\sigma}^2}{p(s')},
    \end{align*}
    where (a) holds by Cauchy inequality and (b) holds by Assumption~\ref{assump: coverage}. Thus, for any vector $\bm{\beta}\in\RB^d$ and $\|\bm{\beta}\|_2=1$, we have:
    \begin{align*}
        \bm{\beta}^\top\sum_{s'\in\SM}\bm{\Delta}(s')^{-1}\bm{\beta}\le\sum_{s'\in\SM}\frac{p(s')}{\underline{\sigma}^2}=\frac{1}{\underline{\sigma}^2}.
    \end{align*}
    Thus, by $V_{\pi^e}(s')\in[0,1/(1-\gamma)]$, we can bound $\var(\psi_{\text{eff},2})$ by
    \begin{align*}
        \var(\psi_{\text{eff},2})\le\frac{1}{\underline{\sigma}^2(1-\gamma)^4}.
    \end{align*}
\end{rem}
